Generative Modeling with Multi-Instance Reward Learning for E-commerce Creative Optimization

In e-commerce advertising, selecting the most compelling combination of creative elements -- such as titles, images, and highlights -- is critical for capturing user attention and driving conversions. However, existing methods often evaluate creative components individually, failing to navigate the exponentially large search space of possible combinations. To address this challenge, we propose a novel framework named GenCO that integrates generative modeling with multi-instance reward learning. Our unified two-stage architecture first employs a generative model to efficiently produce a diverse set of creative combinations. This generative process is optimized with reinforcement learning, enabling the model to effectively explore and refine its selections. Next, to overcome the challenge of sparse user feedback, a multi-instance learning model attributes combination-level rewards, such as clicks, to the individual creative elements. This allows the reward model to provide a more accurate feedback signal, which in turn guides the generative model toward creating more effective combinations. Deployed on a leading e-commerce platform, our approach has significantly increased advertising revenue, demonstrating its practical value. Additionally, we are releasing a large-scale industrial dataset to facilitate further research in this important domain.

==> reproducibility.tex <==
\section{Reproducibility Guidelines}

Unless specified otherwise, please answer ``yes'' to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

This paper:
\begin{itemize}
    \item 
    Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes})
    \item
    Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{yes})
    \item
    Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{yes})
\end{itemize}


Does this paper make theoretical contributions? (\textbf{no})

If yes, please complete the list below.

\begin{itemize}
    \item 
    \item
    All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item
    Proofs of all novel claims are included. (yes/partial/no)
    \item
    Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item
    Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item
    All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item
    All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

Does this paper rely on one or more datasets? (\textbf{yes})

If yes, please complete the list below.

\begin{itemize}
    \item 
    A motivation is given for why the experiments are conducted on the selected datasets (\textbf{yes})
    \item
    All novel datasets introduced in this paper are included in a data appendix. (\textbf{yes})
    \item
    All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
    \item
    All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (\textbf{yes})
    \item
    All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (\textbf{yes})
    \item
    All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\textbf{yes})
\end{itemize}

Does this paper include computational experiments? (\textbf{yes})

If yes, please complete the list below.

\begin{itemize}
    \item 
    This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{yes})
    \item
    Any code required for pre-processing data is included in the appendix. (\textbf{yes})
    \item
    All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{yes})
    \item
    All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
    \item
    All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{yes})
    \item
    If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{yes})
    \item
    This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{yes})
    \item
    This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes})
    \item
    This paper states the number of algorithm runs used to compute each reported result. (\textbf{yes})
    \item
    Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{yes})
    \item
    The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).  (\textbf{yes})
    \item
    This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{yes})
\end{itemize}
